Practical Fault-Tolerant Data Aggregation

During Financial Cryptography 2012 Chan et al. presented a novel privacy-protection fault-tolerant data aggregation protocol. Comparing to previous work, their scheme guaranteed provable privacy of individuals and could work even if some number of users refused to participate. In our paper we demonstrate that despite its merits, their method provides unacceptably low accuracy of aggregated data for a wide range of assumed parameters and cannot be used in majority of real-life systems. To show this we use both precise analytic and experimental methods. Additionally, we present a precise data aggregation protocol that provides provable level of security even facing massive failures of nodes. Moreover, the protocol requires significantly less computation (limited exploiting of heavy cryptography) than most of currently known fault tolerant aggregation protocols and offers better security guarantees that make it suitable for systems of limited resources (including sensor networks). To obtain our result we relax however the model and allow some limited communication between the nodes.

==> img/nodesending__Kopia_powoduj_ca_konflikty__u_ytkownik_Marek_Klonowski__2016-04-14_.tex <==
\begin{figure}
\centering
\tikzstyle{peers}=[draw,circle,black,bottom color=white,
                  top color= white, text=black,minimum width=10pt]
\tikzstyle{lAgg}=[draw,circle,gray,bottom color=gray, top color=gray,
                       text=white,minimum width=20pt]

 \tikzstyle{myarrow}=[->,>=stealth,font=\scriptsize]
  \tikzstyle{brace}=[decorate,decoration={brace,amplitude=5pt}]
  \begin{tikzpicture}[xscale=0.7,yscale=0.65]
   \begin{scope}

	  \node (t1) [peers] at (2,1.5) {$v_1$};
    \node (t2) [peers] at (2.5,-2) {$v_2$};
    \node (t3) [peers]  at (-0.5,-3) {$v_3$};    
    \node (t4) [peers] at (-3.2,0) {$v_4$};
    \node (t5) [peers] at (-2.85,2.5) {$v_5$};
		\node (v)  [peers] at (0,0) {$v$};
		\node (A)  [lAgg] at (0.75,4) {$\lAgg$};
		\node[ellipse,draw=black,thick,dotted,fit=(A) (v) (t2) (t3) (t1),inner sep=0pt] {};

   \foreach \speer/\peer in {v/t1,v/t2,v/t3, v/t4, v/t5, v/A}
    \path (\speer) edge (\peer);
	\end{scope}%x1

%
 \draw [myarrow] (v) -- (t1)  node[midway,above]{$x^v_{v_1}$};
 \draw [myarrow] (t1) -- (v)  node[midway,below]{$x_v^{v_1}$};
%
%
 \draw [myarrow] (v) -- (t2)  node[midway,above]{$x^v_{v_2}$};
 \draw [myarrow] (t2) -- (v)  node[midway,below]{$x_v^{v_2}$};
%
%
 \draw [myarrow] (v) -- (t3)  node[midway,above]{$x^v_{v_3}$};
 \draw [myarrow] (t3) -- (v)  node[midway,below]{$x_v^{v_3}$};
%
%
 \draw [myarrow] (v) -- (t4)  node[midway,above]{$x^v_{v_4}$};
 \draw [myarrow] (t4) -- (v)  node[midway,below]{$x_v^{v_4}$};
%
%
 \draw [myarrow] (v) -- (t5)  node[midway,above]{$x^v_{v_5}$};
 \draw [myarrow] (t5) -- (v)  node[midway,below]{$x_v^{v_5}$};
%
	
	 \draw [myarrow] (v) -- (A)  node[midway,above right]{$Re(\Enc{\sk+\sk_i}{g^{c_v}})$};
	
	  \end{tikzpicture}
  \caption{An example of communication in a single aggregation round from a perspective of node $v$. The dotted line marks the set of nodes assigned to a single local aggregator $\lAgg$. Note that neighbors may may have different local aggregators. }\label{fig:node}
\end{figure}


==> img/topology__Kopia_powoduj_ca_konflikty__u_ytkownik_Marek_Klonowski__2016-04-14_.tex <==

\tikzstyle{peers}=[draw,circle,black,bottom color=white,
                  top color= white, text=black,minimum width=10pt]
\tikzstyle{lAgg}=[draw,circle,gray,bottom color=gray, top color=gray,
                       text=white,minimum width=20pt]
\tikzstyle{AGG}=[rectangle, rounded corners, thin,
                           black, fill= black, draw, text=white,
                           minimum width=2.5cm, minimum height=0.8cm]
													
\begin{figure}
\centering
\begin{tikzpicture}[auto, thick]
   % Agg
   \node[AGG] (Agg) at (0,4) {\small{$\Agg$}};
  % lAgg
  \foreach \place/\name in {{(-4.5,0.5)/a}, {(2,0)/b}, {(2,2)/c}, {(0,2)/d},
           {(-2,0)/e}}
    \node[lAgg] (\name) at \place {$\lAgg$};
	% lAgg->Agg	
		  \foreach \source in {a, b, c, d, e}
    \path (\source) edge (Agg);
		
   %
   % nodes
	 % e
  \foreach \pos/\i in {above left of/1, left of/2, below left of/3, below of/4}
    \node[peers, \pos = e] (e\i) {};
   \foreach \speer/\peer in {e/e1,e/e2,e/e3, e/e4, e1/e2,e2/e4, e1/e3, e3/e4}
    \path (\speer) edge (\peer);
		
		\node[ellipse,draw=black,thick,dotted,fit=(e) (e1) (e2) (e3) (e4),inner sep=0pt] {};
		
   % b
   \foreach \pos/\i in {above right of/1, right of/2, below right of/3}
    \node[peers, \pos =b ] (b\i) {};
   \foreach \speer/\peer in {b/b1,b/b2,b/b3, b1/b2, b2/b3,b3/b1}
   \path (\speer) edge (\peer);
	
			\node[ellipse,draw=black,thick,dotted,fit=(b) (b1) (b2) (b3),inner sep=0pt] {};
   % d
	 \foreach \pos/\i in {below right of/1, below of/2}
   \node[peers, \pos =d ] (d\i) {};
   \foreach \speer/\peer in {d/d1,d/d2,d1/d2}
   \path (\speer) edge (\peer);
	
			\node[ellipse,draw=black,thick,dotted,fit=(d) (d1) (d2),inner sep=0pt] {};
   % a
   \foreach \pos/\i in {below left of/1, below of/2}
   \node[peers, \pos =a ] (a\i) {};
   \foreach \speer/\peer in {a/a1,a/a2, a2/a1}
   \path (\speer) edge (\peer);
	
			\node[ellipse,draw=black,thick,dotted,fit=(a) (a1) (a2),inner sep=0pt] {};
   % c
   \foreach \pos/\i in {above right of/1, right of/2, above of/3}
   \node[peers, \pos =c ] (c\i) {};
   \foreach \speer/\peer in {c/c1,c/c2, c/c3,c3/c1,c1/c2}
   \path (\speer) edge (\peer);
		\node[ellipse,draw=black,thick,dotted,fit=(c) (c1) (c2) (c3),inner sep=0pt] {};
	%%%inter Agg edges
	   \foreach \speer/\peer in {c2/b1,b2/c2,b1/d1,d2/e4,e2/a2,e3/a2}
   \path (\speer) edge (\peer);
	
\end{tikzpicture}
  \caption{Example of a clusterized network with global aggregator ($\Agg$) and local aggregators ($\lAgg$) marked.}\label{fig:topo}
\end{figure}
